A fast and frugal Gaussian Boson Sampling emulator

If classical algorithms have been successful in reproducing the estimation of expectation values of observables of some quantum circuits using off-the-shelf computing resources, matching the performance of the most advanced quantum devices on sampling problems usually requires extreme cost in terms of memory and computing operations, making them accessible to only a handful of supercomputers around the world. In this work, we demonstrate for the first time a classical simulation outperforming Gaussian boson sampling experiments of one hundred modes on established benchmark tests using a single CPU or GPU. Being embarrassingly parallelizable, a small number of CPUs or GPUs allows us to match previous sampling rates that required more than one hundred GPUs. We believe algorithmic and implementation improvements will generalize our tools to photo-counting, single-photon inputs, and pseudo-photon-number-resolving scenarios beyond one thousand modes. Finally, most of the innovations in our tools remain valid for generic probability distributions over binary variables, rendering it potentially applicable to the simulation of qubit-based sampling problems and creating classical surrogates for classical-quantum algorithms.

==> single_elision.tex <==
\subsection{\label{sec:single_elision}Single Elision Method}

A simplifies version of the sampler expands the probability $p(x_n,\bar{x})$ only up to fourth order ($K=4$) and requires only to compute two approximated marginals: (i) $p^{(+)}(x_{a},\ldots,x_{b})$ containing all variables between $x_a$ and $x_b$; (ii) $p^{(1)}\pars{x_{c},\ldots,\widetilde{x}_i,\ldots,x_1}$, with all variables between $x_{c}$ and $x_1$ except for one elision at $x_i$. This approximation is significantly faster to generate samples from, but is not able to outperform all experiments, as discussed in the manuscript. 
The expansion of the probability $p(x_n,\bar{x})$ of the single elision approximation reads:
\begin{eqnarray} \label{eq:probade}
    p(x_n,...,x_1) &=& \frac{1}{2} \pars{1+\mu_{\braces{n}}}\, p(x_{n-1},\ldots,x_1) \nonumber\\ 
    &+& \frac{1}{4} \sum_{i=0}^{n-1} \mu_{\braces{i,n}}\,p^{(1)}\pars{x_{n-1},\ldots,\widetilde{x}_i,\ldots,x_1} \nonumber\\ 
    &+& \frac{1}{8} \sum_{i=1}^{n-1} \sum_{j=1}^{i-1} \mu_{\braces{i,j,n}}\,
    p^{(+)}(x_{n-1},\ldots,x_{i+1})\,p^{(1)}\pars{x_{i-1},\ldots,\widetilde{x}_j,\ldots,x_1} \nonumber\\ 
    &+& \frac{1}{16} \sum_{i=0}^{n-1} \sum_{j=1}^{i-1} \sum_{k=1}^{j-1} \mu_{\braces{i,j,k,m}}\,
    p^{(+)}(x_{n-1},\ldots,x_{i+1})\,p^{(+)}(x_{i-1},\ldots,x_{j+1})\,p^{(1)}\pars{x_{j-1},\ldots,\widetilde{x}_k,\ldots,x_1}. 
\end{eqnarray}

At every step there is $1$ terms $p(x_n,...,x_1)$ to compute consisting of a large sum of size 
$\binom{n-1}{3}_{\sum}\approx O(n^3)$. The largest sum update is of order $O(M^3)$, and
its total computing time $\sum_{i=1}^M\binom{i-1}{3}_{\sum} \approx O(M^4)$ operations, requiring only a memory storage of $O(M)$. This does not finalize the cost analysis, as we need to incorporate the cost of the approximated marginals that we details below and we finalize the section with a summary of the total costs.

{\color{red}Raul - Tom, is this paragraph OK? (same comments as for double-elision)}
As we will see below a key aspect of the design of the approximated marginals is to 
ensure the cost of filling the tables corresponding to the approximated marginals do not degrade the asymptotic scaling of $O(n^3)$ for the $n$-th time step and a final time asymptotic of $O(M^4)$. 
This is achieved a the cost of storing $O(M^2)$ tableau data along the dynamical program, a negligeable cost compared to the $\binom{M}{4}\approx O(M^4)$ requirement of storing the cumulants up to order $K=4$.



\subsubsection{Marginal with free last variable}

The approximated marginals $p^{(+)}(x_{n},\ldots,x_{l})$ containing all variables between $x_{n}$ and $x_{l}$ being present is approximated by the following update rule:

\begin{eqnarray} \label{eq:probpartialade}
p^{(+)}(x_n,\ldots,x_\ell) &=& \frac{1}{2} \pars{1+\mu_{\braces{n}}}\, p^{(+)}(x_{n-1},\ldots,x_\ell) \nonumber\\ 
&+& \frac{1}{4} \sum_{i=\ell}^{m-1} \mu_{\braces{i,n}}\,p^{(+)}\pars{x_{n-1},\ldots,x_{i+1}}\,p^{(+)}\pars{x_{i-1},\ldots,x_\ell} \nonumber\\ 
&+& \frac{1}{8} \sum_{i=\ell}^{n-2} \sum_{j=i+1}^{n-1} \mu_{\braces{i,j,n}}\,p^{(+)}\pars{x_{n-1},\ldots,x_{j+1}}\,p^{(+)}\pars{x_{j-1},\ldots,x_{i+1}}\,p^{(+)}\pars{x_{i-1},\ldots,x_\ell}
\end{eqnarray}

At every step there are $n-1$ terms $p^{(+)}(x_n,\ldots,x_\ell)$ to compute, as $l\in[1,n-1]$:
\begin{itemize}
    \item Each term consist of a large sum of size $\binom{n-1}{2}_{\sum}\approx n^2/2$ of multiplications of 2 or 3 terms.
    \item A total of $3(n-1)\binom{n-1}{2}_{\sum} \approx O(n^3)$ computing operations. 
\end{itemize}

In the process of generating a sample of size $M$ we will need:
\begin{itemize}
    \item a tableau of total size$\sum_{i=1}^M(i-1) \approx M^2$ terms
    \item the longest update take a time $(M-1)\binom{M-1}{2}_{\sum} \approx O(M^3)$
    \item the total computing time $\sum_{i=1}^M (i-1)\binom{i-1}{2}_{\sum} \approx O(M^4)$ operations
\end{itemize}


\subsubsection{Marginal with one elided variable}

The marginals $p^{(1)}\pars{x_{n},\ldots,\widetilde{x}_i,\ldots,x_0}$
with all variables between $x_{n}$ and $x_{0}$ being present except for the elided variable
$x_e$ of index $e\in\{1,n-1\}$ can be computed from the following update rule:

\begin{eqnarray} \label{eq:probelidedade}
    p^{(1)}(x_n,\ldots,\widetilde{x}_{e},\ldots,x_0) &=& \frac{1}{2} \pars{1+\mu_{\braces{n}}}\, p^{(1)}(x_{n-1},\ldots,\widetilde{x}_e,\ldots,x_1) \nonumber\\ 
    &+& \frac{1}{4} \sum_{i=1}^{n-1}\mu_{\braces{i,n}}\,
    p^{(+)}\pars{x_{n-1},\ldots,x_{i+1}} 
    p^{(1)}\pars{x_{i-1},\ldots,\widetilde{x}_b,\ldots,x_1} \nonumber\\ 
    &+& \frac{1}{8} \sum_{\substack{(i\geq j)\in\{1,n-1\}\setminus\{e\}\\ (a,b,c)={\rm ord}(i,j,e)}} 
    \mu_{\braces{i, j, n}}\,p^{(+)}\pars{x_{n-1},\ldots,x_{a+1}} p^{(+)}\pars{x_{a-1},\ldots,x_{b+1}} 
    p^{(1)}\pars{x_{b-1},\ldots,\widetilde{x}_c,\ldots,x_1} \nonumber \\
\end{eqnarray}

 

At every step there are $n-1$ terms $p^{(1)}(x_m,\ldots,\widetilde{x}_{\epsilon},\ldots,x_0)$ to compute, one for each value of the elided variable $e\in[1,n-1]$:
\begin{itemize}
    \item Each term consist of a large sum of size $\binom{n-1}{2}_{\sum}\approx n^2/2$ of multiplications of 2 or 3 terms.
    \item A total of $3(n-1)\binom{n-1}{2}_{\sum} \approx O(n^3)$ computing operations. 
\end{itemize}

In the process of generating a sample of size $M$ we will need:
\begin{itemize}
    \item a tableau of total size $\sum_{i=1}^M(i-1) \approx O(M^2)$ terms
    \item the longest update take a time $(M-1)\binom{M-1}{2}_{\sum} \approx O(M^3)$
    \item the total computing time $\sum_{i=1}^m (i-1)\binom{i-1}{2}_{\sum} \approx O(M^4)$ operations
\end{itemize}

\subsubsection{Total cost estimates}

{\color{red} RAUL - Tom, I think you raised something about the tables...}
In the following table the summarize the information presented above related to the cost of storing and computing the approximated marginals $p^{(+)}$, $p^{(1)}$, $p^{(2)}$ and the sampling distribution $p$ for an $n$-th step of the chain rule and the generation of a single samle of size $M$. Finally, we also give the order on the expansion in terms cumulants for each one. 

\begin{center}
\begin{tabular}{ |c|c|c|c| } 
 \hline
Aux. Marg. & $p^{(+)}$ & $p^{(1)}$  & $p$ \\ 
\hline
 One step &  &  &  \\ 
\hline
Terms & $O(n)$ & $O(n)$  & 1 \\ 
Time/term & $O(n^2)$ & $O(n^2)$  & $O(n^3)$ \\ 
Time & $O(n^3)$ & $O(n^3)$  &  - \\  
\hline
Per sample &  &  &  \\ 
\hline
Memory & $O(M^2)$ & $O(M^2)$  & $O(M)$ \\ 
Longest update & $O(M^3)$ & $O(M^3)$  & $O(M^3)$ \\ 
Total time & $O(M^4)$ & $O(M^4)$  & $O(M^4)$ \\ 
\hline
Exp. Order & 3 & 3  & 4  \\
\hline
\end{tabular}
\end{center}
